Knowledge Guided Representation Learning and Causal Structure Learning in Soil Science

An improved understanding of soil can enable more sustainable land-use practices. Nevertheless, soil is called a complex, living medium due to the complex interaction of different soil processes that limit our understanding of soil. Process-based models and analyzing observed data provide two avenues for improving our understanding of soil processes. Collecting observed data is cost-prohibitive but reflects real-world behavior, while process-based models can be used to generate ample synthetic data which may not be representative of reality. We propose a framework, knowledge-guided representation learning, and causal structure learning (KGRCL), to accelerate scientific discoveries in soil science. The framework improves representation learning for simulated soil processes via conditional distribution matching with observed soil processes. Simultaneously, the framework leverages both observed and simulated data to learn a causal structure among the soil processes. The learned causal graph is more representative of ground truth than other graphs generated from other causal discovery methods. Furthermore, the learned causal graph is leveraged in a supervised learning setup to predict the impact of fertilizer use and changing weather on soil carbon. We present the results in five different locations to show the improvement in the prediction performance in out-of-sample and few-shots setting.

==> ecosys.tex <==
\paragraph{Observed dataset Minnesota}
This dataset contains N\textsubscript{2}O  flux and corresponding environment observations during 2016-2018 growing seasons (i.e., April 1st to July 31st) from six chambers in a controlled-environment mesocosm facility at the University of Minnesota. Soil samples were sourced in 2015 from a farm in Goodhue County, MN, which had been under corn-soybean rotation for 25 years. Six chambers were used to plant continuous corn and monitor the N\textsubscript{2}O flux response to different precipitation treatments. The observed variables include N\textsubscript{2}O flux, CO\textsubscript{2} flux, air temperature, precipitation, radiation, N fertilizer application, crop planting information, and soil properties including soil NO\textsubscript{3}\textsuperscript{-} concentration, NH\textsubscript{4}\textsuperscript{+} concentration, and water content. The details of the mesocosm experiments can be found in ~\cite{MillerEcosys} and the preprocessing setup is similar to ~\cite{gmd-15-2839-2022}.

\paragraph{Simulator \textit{ecosys}}
The \textit{ecosys} model is an advanced agroecosystem model constructed from detailed biophysical and biogeochemical rules instead of using empirical relations~\cite{gmd-15-2839-2022}. It represents N\textsubscript{2}O evolution in the microbe-engaged processes of nitrification-denitrification using substrate kinetics that are sensitive to soil nitrogen availability, soil temperature, soil moisture, and soil oxygen status~\cite{GrantPattyEcosys}. The \textit{ecosys} model was used to generate the synthetic data for the Minnesota site (six experiments from 2016-2018). The input data used to drive these simulations include hourly meteorological (NLDAS-2), layerwise soil properties (gSSURGO database), and the same crop/fertilizer setup as the Minnesota site. The model outputs include N\textsubscript{2}O flux and 76 selected intermediate variables (e.g. CO\textsubscript{2} flux, layerwise soil water content, and soil nitrogen concentration), covering all variables observed in the Minnesota site.

% \paragraph{References} 
% Miller, L. T., Griffis, T. J., Erickson, M. D., Turner, P. A., Deventer, M. J., Chen, Z., Yu, Z., Venterea, R. T., Baker, J. M., & Frie, A. L. (2022). Response of nitrous oxide emissions to individual rain events and future changes in precipitation. In Journal of Environmental Quality (Vol. 51, Issue 3, pp. 312–324). Wiley. https://doi.org/10.1002/jeq2.20348
% Liu, L., Xu, S., Tang, J., Guan, K., Griffis, T. J., Erickson, M. D., Frie, A. L., Jia, X., Kim, T., Miller, L. T., Peng, B., Wu, S., Yang, Y., Zhou, W., Kumar, V., & Jin, Z. (2022). KGML-ag: a modeling framework of knowledge-guided machine learning to simulate agroecosystems: a case study of estimating N&amp;lt;sub&amp;gt;2&amp;lt;/sub&amp;gt;O emission using data from mesocosm experiments. In Geoscientific Model Development (Vol. 15, Issue 7, pp. 2839–2858). Copernicus GmbH. https://doi.org/10.5194/gmd-15-2839-2022
% Grant, R. F.: A review of the Canadian ecosystem model ecosys: Modeling Carbon and Nitrogen Dynamics for Soil Management, 1st edn., CRC Press, Boca Raton, FL, USA, 173–264, ISBN 1566705290, 2001.
% Grant, R. F. and Pattey, E.: Temperature sensitivity of N2O emissions from fertilized agricultural soils: Mathematical modeling in ecosys, Global Biogeochem. Cy., 22, GB4019, https://doi.org/10.1029/2008GB003273, 2008. 

==> introduction_v2.tex <==
In scientific communities, process-based models are often used to study engineered or natural systems. These process-based models integrate physical equations and domain knowledge to capture the complex interaction among physical processes in a system. Therefore, they have also been employed to simulate data, augment input data for machine learning methods and pre-train machine learning models. Despite their extensive use, process-based models heavily rely on calibration of large number of parameters, before they can be employed to study a physical system. Therefore, these models are constrained by their enormous computational costs. Moreover, the calibration process may further be limited by the observed data used. Limited or noisy data may introduce bias or may lead to overfitting in these models. Process-based models also make simplifying assumptions about physical relationships due to incomplete or obsolete knowledge about the physical system. This may further introduce bias in the outputs of the model. 

Machine learning (ML) models , are an alternate, that have found tremendous success in commercial applications. Recently, these methods have increasingly been adopted by domain experts in scientific communities for improving understanding about real-world processes~\cite{dlphysics}. Although ML methods have demonstrated an improved ability in prediction tasks ~\cite{nguyen2021predicting, padarian2020machine}, the reliance of conventional ML on the i.i.d. assumption that training data represents the deployed environment, limits their out-of-distribution generalizability~\cite{ wadoux2020machine, padarian2020machine,  grunwald2022artificial, emadi2020predicting, ren2022dice}. To improve this, either large-scale, diverse data sets are utilized or careful architectural modifications help in better emulation of real-world physical systems. Architectural modifications themselves are limited by domain experts' understanding of the physical system~\cite{lavin2021simulation}. Adopting causal structure learning methods is one approach to overcoming this limitation as these frameworks provide data-driven methods to model cause-and-effect relations among the physical processes explicitly to improve the out-of-distribution generalizability. However, causal structure learning methods make several assumptions that may limit their applicability on real world datasets.  


In this paper, %we consider the problem of out-of-distribution generalization by learning the underlying cause-and-effect relationships. 
we propose a causal structure learning method, Knowledge-Guided Representation learning and Causal Learning (KGRCL), that enables the learning of causal structures from multiple data modalities. In this study, we implement this framework to learn multiple modalities from simulated and observed data, where both datasets provide heterogeneous sources of information about the same underlying processes. This joint modeling allows us to learn richer representations of complex systems by (a) incorporating observed data to mitigate the simplifying modeling assumptions of simulators, and (b) utilizing simulated data to overcome data sparsity which is commonly encountered in observed datasets. Simulated data also offers avenues to learn system characteristics that may be unobserved or difficult to observe. However, often times, data generated by simulators may reflect the assumptions encoded in the simulator and may be biased if the simulator parameters were not calibrated. To overcome these issues, we use conditional distribution matching to improve the learned simulated data representations. 

We present three case studies on soil organic carbon modeling using data from farms located in the UK and the USA. Soil organic carbon (SOC) is the carbon component of organic compounds found in soil both as biomass and as sequestered compounds and necromass. Studying  SOC is of great significance because it is considered as a ``natural insurance against climate change'' \cite{droste2020soil}---with evidence associating increased soil organic matter with increased crop yields~\cite{SCHJONNING201835, soil-5-15-2019, Lal27A}. Proper management of soil, including its organic carbon component, can mitigate shortages in food, water, energy and adverse repercussions of climate change~\cite{de2016towards}.  This has led to increased interest by environmentalists, economists and soil scientists, as interdisciplinary collaborations, in improving public awareness and policy making \cite{lal2004managing, nziguheba2015soil, white2005principles, bhattacharyya2015soil, minasny2017soil, lal2004soil}.
 %This cyclical relationship between soil organic carbon changes and climate change also allows soil organic carbon to potentially help mitigate climate-change-driven problems. 
While the problem of studying soil organic carbon is well-motivated, forming hypotheses and designing experiments to estimate soil organic carbon can be challenging. Changes in soil organic carbon are not only dictated by weather events and management practices, but also by other soil processes such as plant nutrient uptake, soil organisms, soil texture, micro-nutrient content and soil disturbance. This makes soil a complex ``living'' porous medium \cite{de2014soil, de2016towards, ohlson2014soil}. %Thus a simplified study focusing on only a subset of these soil processes may lead to biased soil organic carbon estimates. 
Due to the complex nature of soil science, the exact relations among all soil processes is not yet known. There is no accepted universal method for studying soil organic carbon and the relation among soil processes \cite{bouma2002land}. Moreover, current models of soil organic carbon (RothC-26.3~\cite{rothc}, Century~\cite{century}, DNDC~\cite{GILTRAP2010292}, and some inter-model comparisons \cite{palosuo2012multi, tupek2019evaluating, todd2013causes, smith2012crop}) are not consistent with the latest advances in understanding of soil processes and do not generalize to different soil conditions found globally as they are limited by their modeling assumptions\cite{modelingsoilprocesses}. Therefore, generalizable ML methods can be pivotal in standardizing efforts for soil carbon measuring, reporting and verification across different regions, soil conditions and land use types.

We summarize our key contributions below:

\begin{itemize}
    \item We propose a causal structure learning and representation learning method that jointly models heterogenous sources of data. In our experiments, we utilize observed data and simulated data to learn the causal structure and representations on the input data. Our causal structure learning experiments show that KGRCL outperforms other causal discovery methods and provides improved representations of the simulated data. 
    \item We validate the effectiveness of the proposed framework through extensive experiments on multiple case studies in soil sciences.  For these experiments, we include widely-used process models for simulating soil carbon and other soil processes~\cite{li1996dndc, gmd-15-2839-2022}.
    \item Consequently, we use the learned causal structure in out-of-distribution prediction tasks for soil carbon estimation. 
\end{itemize}

 
